GetMesh: A Controllable Model for High-quality Mesh Generation and Manipulation

Mesh is a fundamental representation of 3D assets in various industrial applications, and is widely supported by professional softwares. However, due to its irregular structure, mesh creation and manipulation is often time-consuming and labor-intensive. In this paper, we propose a highly controllable generative model, GetMesh, for mesh generation and manipulation across different categories. By taking a varying number of points as the latent representation, and re-organizing them as triplane representation, GetMesh generates meshes with rich and sharp details, outperforming both single-category and multi-category counterparts. Moreover, it also enables fine-grained control over the generation process that previous mesh generative models cannot achieve, where changing global/local mesh topologies, adding/removing mesh parts, and combining mesh parts across categories can be intuitively, efficiently, and robustly accomplished by adjusting the number, positions or features of latent points. Project page is https://getmesh.github.io.

==> tables/1NN_CD.tex <==
\begin{table}[h]
\centering
\scalebox{0.9}{
\begin{tabular}{l|cccc}
    \toprule[1.5pt]
    Method& Airplane & Car & Chair & Table\\
    \midrule[1pt]
    SDF-StyleGAN~\cite{zheng2022sdf} & 88.10 & 95.20 & 65.22 & 75.18\\
    NFD~\cite{Shue20223DNF} & 72.00 & 86.70 & 56.36 & - \\
    GET3D~\cite{Gao2022GET3DAG} & - & 97.00 & 68.97 & 68.37\\
    MeshDiffusion~\cite{Liu2023MeshDiffusionSG} & 73.60 & 89.20 & 67.77 & 57.81\\
    SLIDE~\cite{lyu2023controllable} &80.20 & 91.95 & 59.41 & -\\
    3DILG~\cite{Zhang20223DILGIL} & 85.20 & 95.25 & 74.27 & 82.43\\
    Ours & \textbf{70.70} & \textbf{85.35} & \textbf{53.00} & \textbf{53.90} \\
    \bottomrule[1.5pt]
\end{tabular}
}
\caption{1-NNA (CD) comparison between our method and baselines. ``-'' indicates that no checkpoint is provided for that category.}
\label{table: 1_nna_cd}
\end{table}


==> tables/1NN_EMD.tex <==
\begin{table}[h]
\centering
\scalebox{0.9}{
\begin{tabular}{l|cccc}
    \toprule[1.5pt]
    Method& Airplane & Car & Chair & Table\\
    \midrule[1pt]
    SDF-StyleGAN~\cite{zheng2022sdf} &91.75 & 94.65 & 70.27 & 75.08\\
    NFD~\cite{Shue20223DNF} & 79.30 & 88.30 & 57.20 & - \\
    GET3D~\cite{Gao2022GET3DAG} & - & 92.90 & 65.16 & 67.76\\
    MeshDiffusion~\cite{Liu2023MeshDiffusionSG} &74.60 & 88.10 & 67.86 & 60.21\\
    SLIDE~\cite{lyu2023controllable} &80.25 & 92.55 & 61.01 & -\\
    3DILG~\cite{Zhang20223DILGIL} & 88.15 & 94.30 & 73.62 & 81.43\\
    Ours & \textbf{68.80} & \textbf{82.50} & \textbf{52.85} & \textbf{54.35} \\
    \bottomrule[1.5pt]
\end{tabular}
}
\caption{1-NNA (EMD) comparison between our method and baselines. ``-'' indicates that no checkpoint is provided for that category.}
\label{table: 1_nna_emd}
\end{table}

==> tables/ablation_1nna_emd.tex <==
\begin{table}[h]
\centering
\scalebox{1}{
\begin{tabular}{cc|cccc}
    \toprule[1.5pt]
    $N_{\text{min}}$ & $N_{\text{max}}$ & Airplane & Car & Chair & Table\\
    \midrule[1pt]
    % Ours ($N\in [32, 64]$) old & 74.50 & 88.90 & 55.51 & 54.10 \\
    32 & 64 & 94.90 & 90.00 & 83.68 & 85.19 \\
    128 & 256 & \textbf{68.80} & \textbf{82.50} & \textbf{52.85} & \textbf{54.35} \\
    512 & 1024 & 74.85 & 84.60 & 76.03 & 75.23 \\
    2048 & 4096 & 99.90 & 99.70 & 99.34 & 98.59 \\
    \bottomrule[1.5pt]
\end{tabular}
}
\caption{1-NNA (EMD) comparison among our methods with different number of latent points.}
\label{table: abalation_1_nna_emd}
\end{table}
